Towards a Formal Creativity Theory: Preliminary results in Novelty and Transformativeness

Formalizing creativity-related concepts has been a long-term goal of Computational Creativity. To the same end, we explore Formal Learning Theory in the context of creativity. We provide an introduction to the main concepts of this framework and a re-interpretation of terms commonly found in creativity discussions, proposing formal definitions for novelty and transformational creativity. This formalisation marks the beginning of a research branch we call Formal Creativity Theory, exploring how learning can be included as preparation for exploratory behaviour and how learning is a key part of transformational creative behaviour. By employing these definitions, we argue that, while novelty is neither necessary nor sufficient for transformational creativity in general, when using an inspiring set, rather than a sequence of experiences, an agent actually requires novelty for transformational creativity to occur.

==> table_criteria.tex <==

% Criteria table _________________________
\begin{table*}
\caption[Criteria]{Summary of some criteria explored in \gls{flt}\strut}\label{tab:criteria}
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\begin{tabular}{@{} p{5cm} l @{}}
\toprule
\bfseries Criteria's Name & \bfseries\rmfamily Short Explanation \\

\toprule

%Exact & no tolerance \\

\multicolumn{2}{ l }{\textbf{Criteria for Languages}}\\
\midrule
Anomalous Identification & the scientist needs to converge on a finite variant of the correct reality \\
Vacillatory Identification & the scientist can diverge but only inside a finite set of hypotheses for the same reality \\
Behaviourally Correct Identification & the scientist can diverge indefinitely but the hypotheses must all be for the same reality \\
Approximate Identification & the scientist converges to a set which asymptotic disagreement with the reality is bounded\\
\midrule


\multicolumn{2}{ l }{\textbf{Criteria for Classes of Languages}}\\
\midrule
Exact Identification & the scientist does not identify texts for other languages outside a class of languages \\

%Meta & the (meta-)scientist converges to a meta-hypothesis, a computational scientist, which converges to a right hypothesis on the same text \\

\bottomrule
\end{tabular}
\end{table*}


==> table_environments.tex <==

% environments table _________________________
\begin{table*}
\caption[Environments]{Summary of some environments explored in \gls{flt}\strut}\label{tab:environments}
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\begin{tabular}{@{} p{3.5cm} l @{}}
\toprule
\bfseries Environment's Name & \bfseries\rmfamily Short Explanation \\

\toprule
\multicolumn{2}{ l }{\textbf{Data Repetition}}\\
\midrule
Fat Text & the text includes each one of the examples infinitely many times \\
\midrule


\multicolumn{2}{ l }{\textbf{Inaccurate Data}}\\
\midrule
Noisy Data & the text includes some wrong data that should not include \\
Incomplete Data & the text includes all but some of the examples \\
Imperfect Data & the text can miss some examples or have wrong examples that should not be included \\
\midrule


\multicolumn{2}{ l }{\textbf{Data with Additional Structure}}\\
\midrule
Ascending Text & the text presents data sorted in ascending order \\
Recursive Text & the text could have been produced by using a recursive function \\
Nonrecursive Text & the text could not have been produced by using a recursive function \\
Informant & the text includes all possible data, both negative and positive, with notations saying if it is the real set or not \\
Multiple-texts & there are several texts for the same set and the scientist can access them in parallel \\

\bottomrule
\end{tabular}
\end{table*}


==> table_property_criteria.tex <==

% Property Criteria table _________________________
\begin{table*}
\caption[Property based Criteria]{Summary of proposed property based criteria\strut}\label{tab:property_criteria}
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\begin{tabular}{@{} l l l @{}}
\toprule
\bfseries Criteria Designation & \bfseries\rmfamily Short Explanation & Semi-decidable for Non-primitive-recursive $V$ \\

\toprule

%Exact & no tolerance \\

\multicolumn{2}{ l }{\textbf{Single Property Boolean}}\\
\midrule

no $V$-valuable artefacts & there is no artefact $a \in W_{M(\sigma)}$ such that $V(a) = 1$ & No (because of possibly non-terminus of an artefact) \\

$V$-valuable artefacts & there is at least an artefact $a \in W_{M(\sigma)}$ such that $V(a) = 1$ & Yes \\

only $V$-valuable artefacts & every artefact $a \in W_{M(\sigma)}$ also verifies $V(a) = 1$ &  \\

all $V$-valuable artefacts & every artefact $a$ such that $V(a) = 1$ also verifies $a \in W_{M(\sigma)}$ & No (because of possibly non-halting of an enumerator, maybe related to computable identifiable) \\

at least $n$ $V$-valuable artefacts & there are at least $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 1$ & Yes \\

$n$ $V$-valuable artefacts & there are exactly $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 1$ & No (because of possibly non-terminus of an artefact) \\

at most $n$ $V$-valuable artefacts & there are no more than $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 1$ & No (because of possibly non-terminus of an artefact) \\

finitely-many $V$-valuable artefacts & there are no more than $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 1$ & No (because of possibly non-terminus of an artefact) \\

\midrule


no non-$V$-valuable artefacts & there is no artefact $a \in W_{M(\sigma)}$ such that $V(a) = 0$ & Yes \\

non-$V$-valuable artefacts & there is at least an artefact $a \in W_{M(\sigma)}$ such that $V(a) = 0$ & No \\

only non-$V$-valuable artefacts & every artefact $a \in W_{M(\sigma)}$ also verifies $V(a) = 0$ & No \\

all non-$V$-valuable artefacts & every artefact $a$ such that $V(a) = 0$ also verifies $a \in W_{M(\sigma)}$ & Yes \\

at least $n$ $V$-valuable artefacts & there are at least $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 0$ & Yes \\

$n$ $V$-valuable artefacts & there are exactly $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 0$ & No (because of possibly non-terminus of an artefact) \\

at most $n$ $V$-valuable artefacts & there are no more than $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 0$ & No (because of possibly non-terminus of an artefact) \\

\multicolumn{2}{ l }{\textbf{Single Property Parameterized}}\\
\midrule

on average $V$-valuable $\theta$ artefacts & there are no more than $n$ artefacts $a \in W_{M(\sigma)}$ such that $V(a) = 0$ & criterion 1 ritchie\\


\multicolumn{2}{ l }{\textbf{Criteria for Properties }}\\
\midrule

\multicolumn{2}{ l }{\textbf{Scientists Role}}\\
consider & \\
generates & \\
discriminates & \\

\multicolumn{2}{ l }{\textbf{Criteria for Properties }}\\
\midrule
always &  \\
persistently & \\
rarely & \\
never & \\





%Meta & the (meta-)scientist converges to a meta-hypothesis, a computational scientist, which converges to a right hypothesis on the same text \\

\bottomrule
\end{tabular}
\end{table*}


==> table_strategies.tex <==
\begin{table*}
\caption[Strategies]{Summary of some strategies explored in \gls{flt}\strut}\label{tab:strategies}
\centering
\footnotesize
\renewcommand\arraystretch{1.2}
\begin{tabular}{@{} p{3.5cm} l @{}}
\toprule
\bfseries Strategy's Name & \bfseries\rmfamily Short Explanation \\

\toprule
\multicolumn{2}{ l }{\textbf{Regarding Data Invariance}}\\
\midrule
Rearrangement Invariance & the scientist always outputs the same for rearrangements of the prefix, ignoring the order \\
Set-Drivenness &  the scientist always outputs the same for prefixes with the same content, ignoring the order and repetitions \\

\midrule
\multicolumn{2}{ l }{\textbf{Regarding Convergence In The Limit}}\\
\midrule
Order Independence & the scientist converges always to the same hypothesis for texts for the same set \\
Reliability & the scientist does not converge for texts it does not identify \\

\midrule
\multicolumn{2}{ l }{\textbf{Regarding Potential Hypothesis}}\\
\midrule
Totality & the scientist always provides an output for every prefix \\
Consistency & the scientist only provides hypotheses that cover the data that is in the prefix \\
Accountability & the scientist provides hypotheses that predict some data that is still not in the prefix \\
Prudence & the scientist only outputs hypotheses that correspond to realities that it identifies \\

\midrule
\multicolumn{2}{ l }{\textbf{Regarding the Hypotheses' Order}}\\
\midrule
Conservatism & the scientist only changes hypothesis when some data contradicts the previous hypothesis \\
Decisiveness & the scientist never goes back to an abandoned hypothesis \\

\\
\multicolumn{2}{ l }{Generalization Strategies}\\
Strong Monotonicity &  the scientist conjectures sets that never shrink when provided more data \\
Monotonicity & the scientist conjectures sets which intersection with the real set never shrinks when provided more data \\
Weak Monotonicity & the scientist conjectures sets that never shrink unless when provided data that contradicts its previous hypothesis \\ 

\\
\multicolumn{2}{ l }{Specialization Strategies}\\
Dual Strong Monotonicity & the scientist conjectures sets that never grow when provided more data \\
Dual Monotonicity & the scientist conjectures sets which intersection with the real set never grows when provided more data \\
Dual Weak Monotonicity & the scientist conjectures sets that never grow unless when provided data that contradicts its previous hypothesis \\

\midrule
\multicolumn{2}{ l }{\textbf{Regarding Other Aspects}}\\
\midrule
Self-monitorization & the scientist must announce before converging by outputting a special sign \\
Computability & the scientist must be computable/recursive \\
Memory Limitation & the scientist conjectures solely based on the last data point and the previous conjecture \\

\bottomrule
\end{tabular}
\end{table*}


